Safe Sequential Testing and Effect Estimation in Stratified Count Data

Sequential decision making significantly speeds up research and is more cost-effective compared to fixed-n methods. We present a method for sequential decision making for stratified count data that retains Type-I error guarantee or false discovery rate under optional stopping, using e-variables. We invert the method to construct stratified anytime-valid confidence sequences, where cross-talk between subpopulations in the data can be allowed during data collection to improve power. Finally, we combine information collected in separate subpopulations through pseudo-Bayesian averaging and switching to create effective estimates for the minimal, mean and maximal treatment effects in the subpopulations.

==> arXiv versie AISTATS 2023 Safe Sequential Testing/shortcuts/artTheorems.tex <==
% hieronder volgen de settings voor het amsthm-package
% hieronder volgen de settings voor het amsthm-package
\theoremstyle{plain}                          % voor stellingen en zo, die gaan in italics
\newtheorem{thm}{Theorem}[section]     % stellingen worden genummerd volgens de sections
\newtheorem*{hoofdstelling}{Claim}  % een hoofdstelling (zonder nummer)
\newtheorem{lemma}[thm]{Lemma}           % lemma's worden genummerd als stellingen
\newtheorem{proposition}[thm]{Proposition}           % lemma's worden genummerd als stellingen
\newtheorem{eigenschappen}{Properties}
\newtheorem{coro}[thm]{Corollary}
\newtheorem{define}[thm]{Definition}

%\theoremstyle{definition}                     % voor definities en zo, die gaan in romeins font
%\newtheorem{define}[thm]{Definition}   % worden genummerd als de stellingen
\newtheorem{example}[thm]{Example}   % worden genummerd als de stellingen
\newtheorem{remark}[thm]{Remark}            % opmerkingen worden niet genummerd

%\theoremstyle{remark}                         % voor opmerkingen en zo
%\newtheorem{opmerking}[stelling]{Remark}            % opmerkingen worden niet genummerd

% einde settings voor het amsthm-package

% nog wat handige commando's zelf definieren


==> arXiv versie AISTATS 2023 Safe Sequential Testing/shortcuts/shortcuts.tex <==

% LETTERS ---------------------------------------------------------------------------------------------------------
%
\newcommand{\1}{\mathbf{1}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Af}{\mathbb{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Bk}{\mathfrak{B}}
\newcommand{\Bf}{\mathbb{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ck}{\mathfrak{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Df}{\mathbb{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Ef}{\mathbb{E}}
\newcommand{\Ff}{\mathbb{F}}
\newcommand{\Fn}{\mathbb{F}_{n}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Gf}{\mathbb{G}}
\newcommand{\Gn}{\mathbb{G}_{n}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Kf}{\mathbb{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Lf}{\mathbb{L}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Mnc}{\mathcal{M} \mathcal{N}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Nn}{N_{n}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Pf}{\mathbb{P}}
\newcommand{\Pn}{\mathbb{P}_{n}}
\newcommand{\Ps}{\mathscr{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Qf}{\mathbb{Q}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Uf}{\mathbb{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Wf}{\mathbb{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Xf}{\mathbb{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}

% DERIVATIVE ---------------------------------------------------------------------------------------------------
%
\newcommand{\der}{\mathrm{d}}

% DISTRIBUTIONS ----------------------------------------------------------------------------------------------
%
\newcommand{\iid}{\textnormal{iid}}

\newcommand{\Ber}{\textnormal{Ber}}
\newcommand{\Bin}{\textnormal{Bin}}
\newcommand{\Pois}{\textnormal{Pois}}
\newcommand{\Gam}{\textnormal{Gam}}
\newcommand{\Beta}{\textnormal{Beta}}
\newcommand{\SBeta}{\textnormal{SBeta}}
\newcommand{\BetaPrime}{\textnormal{Beta2}}
\newcommand{\Dir}{\textnormal{Dir}}
\newcommand{\IG}{\textnormal{IG}}
\newcommand{\NIG}{\textnormal{NIG}}
\newcommand{\GIG}{\textnormal{GIG}}
\newcommand{\Exp}{\textnormal{Exp}}

% CONVERGENCE ------------------------------------------------------------------------------------------------
%
\newcommand{\as}{\overset{\textnormal{a.s.}}{\rightarrow}}
\newcommand{\inProb}{\overset{P}{\rightarrow}}
\newcommand{\inDist}{\overset{\textnormal{d}}{\rightarrow}}
\newcommand{\isDist}{\overset{\textnormal{d}}{=}}
\newcommand{\iidSim}{\overset{\iid}{\sim}}

% MATRICES -------------------------------------------------------------------------------------------------------
%
\newcommand{\Id}{\textnormal{Id}}
\newcommand{\Span}{\textnormal{Span}}
\newcommand{\tr}{\textnormal{tr}}

\newcommand{\la}{\langle} % Inner product: left
\newcommand{\ra}{\rangle} % Inner product: right

\newcommand{\inn}[2]{ \ensuremath{ \langle #1, #2 \rangle}}

\newcommand{\norm}[1]{ \ensuremath{ \| #1 \| }}
\newcommand{\vecB}[1]{\boldsymbol{#1}}


% OPERATORS -------------------------------------------------------------------------------------------------------
%
\newcommand{\convolution}{\ast}         % convolution
\DeclareMathOperator{\diag}{diag}       % een eigen wiskundeoperator
\DeclareMathOperator{\beeld}{Im}        % eigen wiskundeoperator
\DeclareMathOperator{\vecOp}{vec}
\DeclareMathOperator*{\plim}{plim}

% VARIANCE -----------------------------------------------------------------------------------------------------------
%
\newcommand{\var}{\textnormal{Var}}
\newcommand{\cov}{\textnormal{Cov}}
\newcommand{\cor}{\textnormal{Cor}}

% SUMS OF SQUARES and ERRORS -----------------------------------------------------------------------
%
\newcommand{\rss}{\textnormal{RSS}}
\newcommand{\ess}{\textnormal{ESS}}
\newcommand{\tss}{\textnormal{TSS}}
\newcommand{\mise}{\textnormal{MISE}}

% INFORMATION CRITERIA ---------------------------------------------------------------------------------
%
\newcommand{\Aic}{\textnormal{AIC}}
\newcommand{\Bic}{\textnormal{BIC}}
\newcommand{\Mdl}{\textnormal{MDL}}


% BAYES FACTORS -----------------------------------------------------------------------------
%
\newcommand{\BF}{\textnormal{BF}}
\newcommand{\LR}{\textnormal{LR}}
\newcommand{\info}{\textnormal{info}}
\newcommand{\bc}{\textnormal{BC}}
\newcommand{\elpdLoo}{\textnormal{elpd}_{\textnormal{loo}}}


% Abbreviations --------------------------------------------------------------------------------------------------
%
\newcommand{\dOri}{d_{\textnormal{orig}}}
\newcommand{\dRep}{d_{\textnormal{rep}}}
\newcommand{\dAll}{d_{\textnormal{all}}}

\newcommand{\pOri}{p_{\textnormal{orig}}}
\newcommand{\pRep}{p_{\textnormal{rep}}}

\newcommand{\nAll}{n_{\textnormal{all}}}
\newcommand{\nOri}{n_{\textnormal{orig}}}
\newcommand{\nRep}{n_{\textnormal{rep}}}

\newcommand{\ori}{_{\textnormal{orig}}}
\newcommand{\rep}{_{\textnormal{rep}}}
\newcommand{\all}{_{\textnormal{all}}}

\newcommand{\nPlan}{n_{\textnormal{plan}}}
\newcommand{\mPlan}{m_{\textnormal{plan}}}
\newcommand{\eff}{\textnormal{eff}}


% SPECIAL FUNCTIONS ------------------------------------------------------------------------
%
\newcommand{\sign}{\textnormal{sign}}
\newcommand{\Erf}{\textnormal{Erf}}
\newcommand{\plog}{\textnormal{plog}}
%
\newcommand{\vect}[1]{{\ensuremath{\vec{\reflectbox{\ensuremath{#1}}}}}}

% HYPERGEOMETRIC FUNCTIONS
\newcommand{\iFi}[3]{ \ensuremath{ \, {_{1} F}_{1} \left ( #1 \, ; \,  #2 \, ; \, #3 \right )}}
\newcommand{\iiFi}[4]{ \ensuremath{ \, {_{2} F}_{1} \left ( #1, #2 \, ; \, #3 \, ; \,  #4 \right )}}
\newcommand{\pFq}[7]{ \ensuremath{ \, {_{#1} F}_{#2} \left ( a_{#3}, ..., a_{#4} \, ; \, b_{#5}, ..., b_{#6} \, ; \,  #7 \right )}}
\newcommand{\AFi}[6]{ \ensuremath{ \, AF_{1} \left ( #1 \, ; \,  #2, #3 \, ; \,  #4 \, ; \, #5, #6 \right )}}

% Empirical process
\newcommand{\Gfn}[2]{ \ensuremath{\mathbb{G}_{#1}(#2)}}
% Indicator function
\newcommand{\ind}[1]{\mathbf{1} \left \{ #1 \right \}}

%\definecolor{nOrange}{RGB}{245,160,80}
%\definecolor{nOrange}{RGB}{255,194,10}
%\definecolor{nOrange}{RGB}{255,176,0}
%\definecolor{nBlue}{RGB}{12,123,220}
%\definecolor{nRed}{RGB}{220,50,32}

% COLOURS ------------------------------------------------------------------------------------
%
\definecolor{nRed}{RGB}{220,0,12}
\definecolor{nOrange}{RGB}{254,166,0}
\definecolor{nBlue}{RGB}{40,96,180}

\newcommand{\nRed}[1]{\textcolor{nRed}{#1}}
\newcommand{\nOrange}[1]{\textcolor{nOrange}{#1}}
\newcommand{\nBlue}[1]{\textcolor{nBlue}{#1}}
